Graph Neural Networks as a Substitute for Transformers in Single-Cell Transcriptomics

Graph Neural Networks (GNNs) and Transformers share significant similarities in their encoding strategies for interacting with features from nodes of interest, where Transformers use query-key scores and GNNs use edges. Compared to GNNs, which are unable to encode relative positions, Transformers leverage dynamic attention capabilities to better represent relative relationships, thereby becoming the standard backbones in large-scale sequential pre-training. However, the subtle difference prompts us to consider: if positions are no longer crucial, could we substitute Transformers with Graph Neural Networks in some fields such as Single-Cell Transcriptomics? In this paper, we first explore the similarities and differences between GNNs and Transformers, specifically in terms of relative positions. Additionally, we design a synthetic example to illustrate their equivalence where there are no relative positions between tokens in the sample. Finally, we conduct extensive experiments on a large-scale position-agnostic dataset-single-cell transcriptomics-finding that GNNs achieve competitive performance compared to Transformers while consuming fewer computation resources. These findings provide novel insights for researchers in the field of single-cell transcriptomics, challenging the prevailing notion that the Transformer is always the optimum choice.

==> supp_dict/supp_dataset.tex <==
Single-cell transcriptomics, abbreviated as transcriptomics in the main paper, leverages high-throughput technologies to sequence and analyze RNA from individual cells \cite{kolodziejczyk2015technology}. This method facilitates essential biological tasks such as cell annotation and perturbation prediction. Transcriptomic data typically comprise a sequence-like dataset without positions (\ie, no relative orders between genes), represented as a set of genes and their associated expression values: $(\text{gene}_1, \text{gene}_2, \ldots, \text{gene}_n)$,$ (\text{expr}_1, \text{expr}_2, \ldots, \text{expr}_n)$, where $\text{expr}$ denotes the associated expression values. In transcriptomics, each gene appears only once, and there are no relative orders between genes, \textit{i.e.}, no positions nor relative positions. Due to its sequence-like data structure, many researchers have conducted extensive Transformer-based pretraining on large-scale transcriptomic datasets, consuming significant resources, especially when gene length is extremely large. Therefore, exploring the potential of Graph Neural Networks as an alternative for Transformers in this field, \ie, where the dataset lacks positions, is of significant interest.



We follow the dataset settings and pre-training downstream verification procedure applied in scGPT~\cite{scGPT} to assemble a large-scale transcriptomic dataset for the self-supervised pre-training of our benchmark and five downstream transcriptomic classification datasets. The pre-training dataset comprises single-cell RNA transcriptomics from 54.6 million human cells, which is sourced from the CELLxGENE~\cite{czi2023cz} collection. It includes samples from about 51 organs and tissues (e.g., heart, blood, and brain) derived from more than 441 studies, offering extensive coverage of cellular heterogeneity throughout the human body. The five downstream datasets feature fewer transcriptomic samples but include class labels, such as cell type and disease type, making them suitable for validating the effectiveness of the pre-trained models. Here, we introduce the five transcriptomic datasets in detail:

Leptomeningeal (Lept)~\cite{remsik2023leptomeningeal}, which identifies that leptomeningeal-specific IFN-$\gamma$ signaling plays a pivotal role in cancer cell growth independently of adaptive immunity and suggests a novel immunotherapeutic strategy targeting tumors. This dataset consists of 20,676 cells and includes 10 classes, such as CD4 T cell, CD8 T cell, etc.

Sclerosis~\cite{schirmer2019neuronalMS}, which reveals specific cellular changes in multiple sclerosis lesions, highlighting the roles of neuron damage and glial activation in driving disease progression, which consists of 21,312 cells and 18 classes, such as pyramidal neurons, phagocytes, etc.

Pancreas~\cite{chen2023transformerPanc}, which aggregates data from five human pancreas studies for cell type annotation tasks. This dataset consists of 14,818 cells and includes 14 classes, such as T-cell, ductal, etc.

Lupus~\cite{perez2022single}, which identifies increased type 1 interferon-stimulated genes in monocytes, accompanied by a reduction in naive CD4 T cells and an expansion of cytotoxic GZMH CD8 T cells. This dataset consists of 79,322 cells (we randomly select 50,000 samples among those) and includes 14 classes, such as T4-reg, NK-dim, etc.

Dengue~\cite{ghita2023global}, which identifies the target cells of the dengue virus, including myeloid cells and B cells, and outlines the immunological characteristics of severe dengue progression in children's blood. This dataset consists of 193,727 cells (we randomly select 50,000 samples among those) and includes 23 classes, such as CD8+ naive T cells, CD4+ naive T cells, etc.



==> supp_dict/supp_method.tex <==

\noindent\textbf{Preliminaries.} 

% \smallskip
For the dataset, \eg, trancriptomics, $\mathcal{D}\!=\!\{(\bm{x}_i, \bm{v}_i)\}_{i=1}^N$, where $(\bm{x}_i, \bm{v}_i) = (x_{i,1}, x_{i,2}, \ldots, x_{i,l}; v_{i,1}, v_{i,2}, \ldots, v_{i,l})$. The  masked value input is $(\bm{x}_i, \tilde{\bm{v}}_i) = (x_{i,1}, x_{i,2}, \ldots, x_{i,l}$; $v_{i,1}, [mask], \ldots, v_{i,l})$.
We first re-write the masked value prediction loss, \ie, Eq.~(5) in the main paper, here:
\begin{gather}
\label{supp:base_objective}
\mathcal{L}_{\text{\textit{MVP}}}(\mathcal{D}, \theta) = \frac{1}{N} \sum_{i=1}^N \sum_{k} \left\|v_{i,k} - f((\bm{x}_i, \tilde{\bm{v}}_i), \theta)_k\right\|^2, \tag{a}
\end{gather}
%---------------------------------
where $v_{i,k}$ is the $k$-th masked value in $\tilde{\bm{v}}_i$ and $f((\bm{x}_i, \tilde{\bm{v}}_i), \theta)_k$ represents the corresponding predicted value.

We assume that position \textbf{exists} in this dataset (not the real case in transcriptomics). For the calculation of $f((\bm{x}_i, \tilde{\bm{v}}_i), \theta)_k$, the whole process can be written as:
\begin{gather}
\label{supp:embed_process}
\bm{e} = \mathbf{E_\theta}(\bm{x}_i) + \mathbf{L_{1,\theta}}(\tilde{\bm{v}}_i) + \bm{p}, \tag{b} \\
\label{supp:feature_extraction}
\bm{e}' = (e'_1, e'_2, \ldots, e'_l) = \mathbf{M_\theta}(\bm{e}), \tag{c}\\
\label{supp:value_prediction}
f((\bm{x}_i, \tilde{\bm{v}}_i), \theta)_k = \mathbf{L_{2,\theta}}(e'_k), \tag{d}
\end{gather}
where $\bm{p}=(p_1,p_2,\ldots,p_l)$ is the (absolute) positional embedding and $l$ is the sequence length, other symbols serve as the same roles described in Eq.~(6) to Eq.~(8) in the main paper.

For convenience, we assume there is only one layer of Transformer and GNN, and the feature extraction process for the two models could be re-written as:
\begin{gather}
\bm{e}'_{tf} = \text{\text{Softmax}}\left((\bm{e}\mathbf{w}_Q )(\bm{e}\mathbf{w}_K )^T\right) (\bm{e}\mathbf{w}_V ), \tag{e}\\
\bm{e}'_{gnn} = \text{Softmax}(\mathbf{A}) \bm{e}, \tag{f}
\end{gather}
where the symbols serve the same roles described in Eq.~(9) and Eq.~(11) in the main paper.

\medskip
\noindent\textbf{Comparisons of Empirical Risks.} 
\smallskip

We still apply the assumption in the main paper, that value is defined as the summation of the influence of token, other values, and other values considering relative positions:
\begin{align}
\label{value_gen_func_app}
 v_k = h_1(x_k) + {\textstyle\sum_j} h_2(v_j) + {\textstyle\sum_j} h_3(p_{kj}v_j), \tag{g}
\end{align}
where $h_1$, $h_2$ and $h_3$ are inherent functions for value generation, $j$ indexes all tokens except $k$ in the sample, $p_{kj}$ is the relative positions between $k$ and $j$. Considering the difference between $h_2$ and $h_3$, where the first function aggregates the influence from other values without considering their relative positions. Therefore, when $p_{kj} = 0$ or the influence from associated values $v_j$ to $v_k$ remains constant, $h_3$ effectively performs the same function as $h_2$, \ie, these two functions can be merged. This rationale supports our claim that under certain conditions, function $h_3$ will degenerate to $h_2$ in the main paper.

Assuming that Transformers and GNNs have a similar ability to learn $h_1$ and $h_2$, the difference generated from the training empirical risk (not the generalization risk), Eq.~(14) in the main paper:
\begin{align}
 \mathcal{R}_{h_3} &= {\textstyle\sum_{\mathcal{D}}\sum_j} \|h_3(p_{kj}v_j) - f(p_{kj},v_j)\|^2. \tag{h}
\end{align}

For any two specific tokens $x_k$ and $x_j$, the influence from $x_j$ to $x_k$ varies in response to $p_{kj} \in \mathcal{P}$, encoded by $h_3$, where $\mathcal{P}$ represents the set for all possible values of relative positions. Without loss of generality, by only considering two tokens (the values of $k$ and $j$ could change but tokens $x_k$ and $x_j$ are unchanged) and the effect from $x_j$ to $x_k$ across all samples, $h_3$ as a static coefficient and $g_\theta$ is the optimization target, the risk could be further written as:
\begin{align}
 \mathcal{R}_{h_3,x_j\rightarrow x_k} &= {\textstyle\sum_{\mathcal{D}}} \|h_3p_{kj}v_j - g_\theta v_j\|^2, \tag{i}\\
 &= {\textstyle\sum_{\mathcal{D}}} \|h_3p_{kj} - g_\theta\|^2  \|v_j\|^2. \tag{j}
\end{align}
where $g_\theta$ is the function of $s_{kj}$, where $s_{kj} = (e_k\mathbf{w_Q} ) (e_j\mathbf{w_K} )^T$ for Transformer. Since $e_k$ and $e_j$ encode position $p_k$ and $p_j$ as described in Eq.~\eqref{supp:embed_process}, the optimum for Transformer is $g_\theta^*=h_3(p_k-p_j)=h_3p_{kj}$ and the optimal risk is 0. On the other hand, for GNNs, as its $g_\theta$ does not accept $p_k$ and $p_j$ as input, it can only learn a constant for various $p_{kj}$ from the optimization, and its optimum should be $g_\theta^*=h_3\mathbb{E}\left[p_{kj}\right]$. Given the above discussion, the training risk difference between optimal Transformer and GNN could be written as:
\begin{align}
 \mathcal{R}_{h_3,\Delta} &= {\textstyle\sum_{\mathcal{D}}\sum_j} \|p_{kj} - \mathbb{E}\left[p_{kj}\right]\|^2  \|h_3 v_j\|^2, \tag{k}
\end{align}
where the optimal loss of Transformers is 0 and Eq.~(k) is also the optimal loss for GNN, $\Delta$ denotes the difference between the two models.

Based on the discussions above, we find that if $p_{kj}$ is a constant, (\ie, $p_{kj} = \mathbb{E}\left[p_{kj}\right] = c$, where $c$ is a constant) or even $p_{kj}=0$, the risk difference $\mathcal{R}_{h_3,\Delta}$ is equal to 0, which confirms our hypothesis that Transformers and GNNs are equivalent. To further verify the inherent discrepancy between GNNs and Transformers lies in their ability to handle relative positions, we conducted synthetic experiments and large-scale experiments in the main paper.



==> supp_dict/supp_table.tex <==
\begin{table}[t]
\centering

    \renewcommand{\arraystretch}{1.3}
     \scalebox{0.86}{
\begin{tabular}{c|c|ccccc|c}

\toprule
\(e_p \backslash \sigma\)  &  & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & Avg \\ 
 \hline
\multirow{3}{*}{0} & TF &  0.009 & 0.034 & 0.077& 0.134 & 0.207 & - \\
&GNN         & 0.013 & 0.040 & 0.085 & 0.150 & 0.225 & -\\
& $r_\Delta$  & 1.444 & 1.176 & 1.104 & 1.119 & 1.087 & 1.186 \\
\hline
\multirow{3}{*}{0.1} & TF & 0.010 & 0.030 & 0.069 & 0.119 & 0.217 & - \\
&GNN         & 0.026 & 0.057 & 0.098 & 0.159 & 0.242 & -\\
& $r_\Delta$  & 2.600 & 1.900 & 1.420 & 1.336 & 1.115 & 1.674 \\
\hline
\multirow{3}{*}{0.2} & TF & 0.009 & 0.035 & 0.063 & 0.133 & 0.168& -\\
&GNN         & 0.031 & 0.103 & 0.122 & 0.203 & 0.299 & -\\
& $r_\Delta$  & 3.444 & 2.943 & 1.937 & 1.526 & 1.780 & 2.326\\
\hline
\multirow{3}{*}{0.3} & TF & 0.009 & 0.028 & 0.059 & 0.135 & 0.197 & -  \\
&GNN         & 0.055 & 0.104 & 0.174 & 0.278 & 0.399 & -\\
& $r_\Delta$  & 6.111 & 3.714 & 2.949 & 2.059 & 2.025 & 3.372 \\
\hline
\multirow{3}{*}{0.4} & TF & 0.014 & 0.028 & 0.059 & 0.133 & 0.156 & -\\
&GNN         & 0.096 & 0.166 & 0.269 & 0.406 & 0.584 & -\\
& $r_\Delta$  & 6.857 & 5.929 & 4.559 & 3.053 & 3.744 & 4.828\\
\hline
\multirow{3}{*}{0.5} & TF & 0.017& 0.027 & 0.085 & 0.163& 0.193 & - \\
&GNN         &0.427 & 0.267 & 0.421  &0.621 & 0.884 & - \\
& $r_\Delta$  & 25.12 &9.889 & 4.953& 3.812 & 4.580 & 9.670\\
\bottomrule
\end{tabular}
}
\caption{Supplementary for Table~1 in the main paper where more experimental results across different $e_p$ are provided. Comparisons of test losses in synthetic example between Transformers and GNNs with varying $e_p$ and $\sigma$. $r_\Delta\!=\! \mathcal{L}_{GNN}/\mathcal{L}_{TF}$ indicates the relative loss differences between them. Avg denotes the averaged result across $\sigma$. For $r_\Delta$, a larger number denotes Transformer is better, and for others, a smaller number is better.}
\label{supp:toy_table}
% \vspace{-8pt}
\end{table}

==> supp_dict/supp_table2.tex <==
\begin{table}[t]
\centering
\caption{Supplementary for Table~1 in the main paper with \textbf{no positional encoding} settings, \ie, $\alpha=0$ in Eq.~(15) in the main paper, note that such setting is only a synthetic setting and unlikely to occur in real data. Comparisons of test losses in synthetic example between Transformers and GNNs with varying $e_p$ and $\sigma$. $r_\Delta\!=\! \mathcal{L}_{GNN}/\mathcal{L}_{TF}$ indicates the relative loss differences between them. Avg denotes the averaged result across $\sigma$. For $r_\Delta$, a larger number denotes Transformer is better, and for others, a smaller number is better.}
    \renewcommand{\arraystretch}{1.1}
     \scalebox{1.0}{
\begin{tabular}{c|c|ccccc|c}

\toprule
\(e_p \backslash \sigma\)  &  & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 & Avg \\ 
 \hline
\multirow{3}{*}{0} & TF & 0.009 & 0.034 & 0.075 & 0.136 & 0.208 & -   \\
&GNN         &  0.013 & 0.039 & 0.083 & 0.145 & 0.224 & -\\
& $r_\Delta$  & 1.444 & 1.147 & 1.107 & 1.066 & 1.077 & 1.168 \\
\hline
\multirow{3}{*}{0.1} & TF & 0.008 & 0.033 & 0.068 & 0.119 & 0.186 & -\\
&GNN         & 0.024 & 0.054 & 0.097 & 0.162 & 0.248 & -\\
& $r_\Delta$  & 3.000 & 1.636 & 1.426 & 1.361 & 1.333 & 1.752 \\
\hline
\multirow{3}{*}{0.2} & TF & 0.009 & 0.027 & 0.063 & 0.134 & 0.205 & - \\
&GNN         &0.037 & 0.071 & 0.128 & 0.205 & 0.298 & - \\
& $r_\Delta$  &4.111 & 2.630 & 2.032 & 1.530 & 1.454 & 2.351 \\
\hline
\multirow{3}{*}{0.3} & TF &  0.015 & 0.030 & 0.064 & 0.139 & 0.199 & - \\
&GNN         & 0.073 & 0.112 & 0.185 & 0.280 & 0.407 & -\\
& $r_\Delta$  & 4.867 & 3.733 & 2.891 & 2.014 & 2.045 & 3.110 \\
\hline
\multirow{3}{*}{0.4} & TF& 0.016 & 0.031 & 0.057 & 0.136 & 0.194 & - \\
&GNN         & 0.124 & 0.180 & 0.282 & 0.420 & 0.589 & -\\
& $r_\Delta$  & 7.750 & 5.806 & 4.947 & 3.088 & 3.036 & 4.926 \\
\hline
\multirow{3}{*}{0.5} & TF& 0.012 & 0.050 & 0.089 & 0.133 & 0.191 & -\\
&GNN         &0.206 & 0.297 & 0.439 & 0.621 & 0.882 & - \\
& $r_\Delta$  &17.167 & 5.940 & 4.933 & 4.669 & 4.618 & 7.465 \\
% \hline

\bottomrule
\end{tabular}
}

\label{supp:toy_table_no_pos}
% \vspace{-8pt}
\end{table}
